Model-independent observation of exotic contributions to $B^0\to J/\psi K^+\pi^-$ decays

An angular analysis of $B^0\to J/\psi K^+\pi^-$ decays is performed, using proton-proton collision data corresponding to an integrated luminosity of 3~${\rm fb}^{-1}$ collected with the LHCb detector. The $m(K^+\pi^-)$ spectrum is divided into fine bins. In each $m(K^+\pi^-)$ bin, the hypothesis that the three-dimensional angular distribution can be described by structures induced only by $K^\ast$ resonances is examined, making minimal assumptions about the $K^+\pi^-$ system. The data reject the $K^\ast$-only hypothesis with a large significance, implying the observation of exotic contributions in a model-independent fashion. Inspection of the $m(J/\psi\pi^-)$ versus $m(K^+\pi^-)$ plane suggests structures near $m(J/\psi\pi^-)=4200$~MeV and 4600~MeV.

==> LHCb_Authorship_flat_02-Oct-2018.tex <==
\centerline{\large\bf LHCb collaboration}
\begin{flushleft}
\small
R.~Aaij$^{28}$,
C.~Abell{\'a}n~Beteta$^{46}$,
B.~Adeva$^{43}$,
M.~Adinolfi$^{50}$,
C.A.~Aidala$^{78}$,
Z.~Ajaltouni$^{6}$,
S.~Akar$^{61}$,
P.~Albicocco$^{19}$,
J.~Albrecht$^{11}$,
F.~Alessio$^{44}$,
M.~Alexander$^{55}$,
A.~Alfonso~Albero$^{42}$,
G.~Alkhazov$^{34}$,
P.~Alvarez~Cartelle$^{57}$,
A.A.~Alves~Jr$^{43}$,
S.~Amato$^{2}$,
S.~Amerio$^{24}$,
Y.~Amhis$^{8}$,
L.~An$^{18}$,
L.~Anderlini$^{18}$,
G.~Andreassi$^{45}$,
M.~Andreotti$^{17}$,
J.E.~Andrews$^{62}$,
F.~Archilli$^{28}$,
P.~d'Argent$^{13}$,
J.~Arnau~Romeu$^{7}$,
A.~Artamonov$^{41}$,
M.~Artuso$^{63}$,
K.~Arzymatov$^{38}$,
E.~Aslanides$^{7}$,
M.~Atzeni$^{46}$,
B.~Audurier$^{23}$,
S.~Bachmann$^{13}$,
J.J.~Back$^{52}$,
S.~Baker$^{57}$,
V.~Balagura$^{8,b}$,
W.~Baldini$^{17}$,
A.~Baranov$^{38}$,
R.J.~Barlow$^{58}$,
G.C.~Barrand$^{8}$,
S.~Barsuk$^{8}$,
W.~Barter$^{58}$,
M.~Bartolini$^{20}$,
F.~Baryshnikov$^{74}$,
V.~Batozskaya$^{32}$,
B.~Batsukh$^{63}$,
A.~Battig$^{11}$,
V.~Battista$^{45}$,
A.~Bay$^{45}$,
J.~Beddow$^{55}$,
F.~Bedeschi$^{25}$,
I.~Bediaga$^{1}$,
A.~Beiter$^{63}$,
L.J.~Bel$^{28}$,
S.~Belin$^{23}$,
N.~Beliy$^{66}$,
V.~Bellee$^{45}$,
N.~Belloli$^{21,i}$,
K.~Belous$^{41}$,
I.~Belyaev$^{35}$,
E.~Ben-Haim$^{9}$,
G.~Bencivenni$^{19}$,
S.~Benson$^{28}$,
S.~Beranek$^{10}$,
A.~Berezhnoy$^{36}$,
R.~Bernet$^{46}$,
D.~Berninghoff$^{13}$,
E.~Bertholet$^{9}$,
A.~Bertolin$^{24}$,
C.~Betancourt$^{46}$,
F.~Betti$^{16,44}$,
M.O.~Bettler$^{51}$,
M.~van~Beuzekom$^{28}$,
Ia.~Bezshyiko$^{46}$,
S.~Bhasin$^{50}$,
J.~Bhom$^{30}$,
S.~Bifani$^{49}$,
P.~Billoir$^{9}$,
A.~Birnkraut$^{11}$,
A.~Bizzeti$^{18,u}$,
M.~Bj{\o}rn$^{59}$,
M.P.~Blago$^{44}$,
T.~Blake$^{52}$,
F.~Blanc$^{45}$,
S.~Blusk$^{63}$,
D.~Bobulska$^{55}$,
V.~Bocci$^{27}$,
O.~Boente~Garcia$^{43}$,
T.~Boettcher$^{60}$,
A.~Bondar$^{40,x}$,
N.~Bondar$^{34}$,
S.~Borghi$^{58,44}$,
M.~Borisyak$^{38}$,
M.~Borsato$^{43}$,
F.~Bossu$^{8}$,
M.~Boubdir$^{10}$,
T.J.V.~Bowcock$^{56}$,
C.~Bozzi$^{17,44}$,
S.~Braun$^{13}$,
M.~Brodski$^{44}$,
J.~Brodzicka$^{30}$,
A.~Brossa~Gonzalo$^{52}$,
D.~Brundu$^{23,44}$,
E.~Buchanan$^{50}$,
A.~Buonaura$^{46}$,
C.~Burr$^{58}$,
A.~Bursche$^{23}$,
J.~Buytaert$^{44}$,
W.~Byczynski$^{44}$,
S.~Cadeddu$^{23}$,
H.~Cai$^{68}$,
R.~Calabrese$^{17,g}$,
R.~Calladine$^{49}$,
M.~Calvi$^{21,i}$,
M.~Calvo~Gomez$^{42,m}$,
A.~Camboni$^{42,m}$,
P.~Campana$^{19}$,
D.H.~Campora~Perez$^{44}$,
L.~Capriotti$^{16}$,
A.~Carbone$^{16,e}$,
G.~Carboni$^{26}$,
R.~Cardinale$^{20}$,
A.~Cardini$^{23}$,
P.~Carniti$^{21,i}$,
K.~Carvalho~Akiba$^{2}$,
G.~Casse$^{56}$,
L.~Cassina$^{21}$,
M.~Cattaneo$^{44}$,
G.~Cavallero$^{20}$,
R.~Cenci$^{25,p}$,
D.~Chamont$^{8}$,
M.G.~Chapman$^{50}$,
M.~Charles$^{9}$,
Ph.~Charpentier$^{44}$,
G.~Chatzikonstantinidis$^{49}$,
M.~Chefdeville$^{5}$,
V.~Chekalina$^{38}$,
C.~Chen$^{3}$,
S.~Chen$^{23}$,
S.-G.~Chitic$^{44}$,
V.~Chobanova$^{43}$,
M.~Chrzaszcz$^{44}$,
A.~Chubykin$^{34}$,
P.~Ciambrone$^{19}$,
X.~Cid~Vidal$^{43}$,
G.~Ciezarek$^{44}$,
F.~Cindolo$^{16}$,
P.E.L.~Clarke$^{54}$,
M.~Clemencic$^{44}$,
H.V.~Cliff$^{51}$,
J.~Closier$^{44}$,
V.~Coco$^{44}$,
J.A.B.~Coelho$^{8}$,
J.~Cogan$^{7}$,
E.~Cogneras$^{6}$,
L.~Cojocariu$^{33}$,
P.~Collins$^{44}$,
T.~Colombo$^{44}$,
A.~Comerma-Montells$^{13}$,
A.~Contu$^{23}$,
G.~Coombs$^{44}$,
S.~Coquereau$^{42}$,
G.~Corti$^{44}$,
M.~Corvo$^{17,g}$,
C.M.~Costa~Sobral$^{52}$,
B.~Couturier$^{44}$,
G.A.~Cowan$^{54}$,
D.C.~Craik$^{60}$,
A.~Crocombe$^{52}$,
M.~Cruz~Torres$^{1}$,
R.~Currie$^{54}$,
C.~D'Ambrosio$^{44}$,
F.~Da~Cunha~Marinho$^{2}$,
C.L.~Da~Silva$^{79}$,
E.~Dall'Occo$^{28}$,
J.~Dalseno$^{43,v}$,
A.~Danilina$^{35}$,
A.~Davis$^{3}$,
O.~De~Aguiar~Francisco$^{44}$,
K.~De~Bruyn$^{44}$,
S.~De~Capua$^{58}$,
M.~De~Cian$^{45}$,
J.M.~De~Miranda$^{1}$,
L.~De~Paula$^{2}$,
M.~De~Serio$^{15,d}$,
P.~De~Simone$^{19}$,
C.T.~Dean$^{55}$,
D.~Decamp$^{5}$,
L.~Del~Buono$^{9}$,
B.~Delaney$^{51}$,
H.-P.~Dembinski$^{12}$,
M.~Demmer$^{11}$,
A.~Dendek$^{31}$,
D.~Derkach$^{39}$,
O.~Deschamps$^{6}$,
F.~Desse$^{8}$,
F.~Dettori$^{56}$,
B.~Dey$^{69}$,
A.~Di~Canto$^{44}$,
P.~Di~Nezza$^{19}$,
S.~Didenko$^{74}$,
H.~Dijkstra$^{44}$,
F.~Dordei$^{23}$,
M.~Dorigo$^{44,y}$,
A.~Dosil~Su{\'a}rez$^{43}$,
L.~Douglas$^{55}$,
A.~Dovbnya$^{47}$,
K.~Dreimanis$^{56}$,
L.~Dufour$^{28}$,
G.~Dujany$^{9}$,
P.~Durante$^{44}$,
J.M.~Durham$^{79}$,
D.~Dutta$^{58}$,
R.~Dzhelyadin$^{41}$,
M.~Dziewiecki$^{13}$,
A.~Dziurda$^{30}$,
A.~Dzyuba$^{34}$,
S.~Easo$^{53}$,
U.~Egede$^{57}$,
V.~Egorychev$^{35}$,
S.~Eidelman$^{40,x}$,
S.~Eisenhardt$^{54}$,
U.~Eitschberger$^{11}$,
R.~Ekelhof$^{11}$,
L.~Eklund$^{55}$,
S.~Ely$^{63}$,
A.~Ene$^{33}$,
S.~Escher$^{10}$,
S.~Esen$^{28}$,
T.~Evans$^{61}$,
A.~Falabella$^{16}$,
N.~Farley$^{49}$,
S.~Farry$^{56}$,
D.~Fazzini$^{21,44,i}$,
P.~Fernandez~Declara$^{44}$,
A.~Fernandez~Prieto$^{43}$,
F.~Ferrari$^{16}$,
L.~Ferreira~Lopes$^{45}$,
F.~Ferreira~Rodrigues$^{2}$,
M.~Ferro-Luzzi$^{44}$,
S.~Filippov$^{37}$,
R.A.~Fini$^{15}$,
M.~Fiorini$^{17,g}$,
M.~Firlej$^{31}$,
C.~Fitzpatrick$^{45}$,
T.~Fiutowski$^{31}$,
F.~Fleuret$^{8,b}$,
M.~Fontana$^{44}$,
F.~Fontanelli$^{20,h}$,
R.~Forty$^{44}$,
V.~Franco~Lima$^{56}$,
M.~Frank$^{44}$,
C.~Frei$^{44}$,
J.~Fu$^{22,q}$,
W.~Funk$^{44}$,
C.~F{\"a}rber$^{44}$,
M.~F{\'e}o$^{44}$,
E.~Gabriel$^{54}$,
A.~Gallas~Torreira$^{43}$,
D.~Galli$^{16,e}$,
S.~Gallorini$^{24}$,
S.~Gambetta$^{54}$,
Y.~Gan$^{3}$,
M.~Gandelman$^{2}$,
P.~Gandini$^{22}$,
Y.~Gao$^{3}$,
L.M.~Garcia~Martin$^{76}$,
B.~Garcia~Plana$^{43}$,
J.~Garc{\'\i}a~Pardi{\~n}as$^{46}$,
J.~Garra~Tico$^{51}$,
L.~Garrido$^{42}$,
D.~Gascon$^{42}$,
C.~Gaspar$^{44}$,
L.~Gavardi$^{11}$,
G.~Gazzoni$^{6}$,
D.~Gerick$^{13}$,
E.~Gersabeck$^{58}$,
M.~Gersabeck$^{58}$,
T.~Gershon$^{52}$,
D.~Gerstel$^{7}$,
Ph.~Ghez$^{5}$,
V.~Gibson$^{51}$,
O.G.~Girard$^{45}$,
P.~Gironella~Gironell$^{42}$,
L.~Giubega$^{33}$,
K.~Gizdov$^{54}$,
V.V.~Gligorov$^{9}$,
D.~Golubkov$^{35}$,
A.~Golutvin$^{57,74}$,
A.~Gomes$^{1,a}$,
I.V.~Gorelov$^{36}$,
C.~Gotti$^{21,i}$,
E.~Govorkova$^{28}$,
J.P.~Grabowski$^{13}$,
R.~Graciani~Diaz$^{42}$,
L.A.~Granado~Cardoso$^{44}$,
E.~Graug{\'e}s$^{42}$,
E.~Graverini$^{46}$,
G.~Graziani$^{18}$,
A.~Grecu$^{33}$,
R.~Greim$^{28}$,
P.~Griffith$^{23}$,
L.~Grillo$^{58}$,
L.~Gruber$^{44}$,
B.R.~Gruberg~Cazon$^{59}$,
O.~Gr{\"u}nberg$^{71}$,
C.~Gu$^{3}$,
E.~Gushchin$^{37}$,
A.~Guth$^{10}$,
Yu.~Guz$^{41,44}$,
T.~Gys$^{44}$,
C.~G{\"o}bel$^{65}$,
T.~Hadavizadeh$^{59}$,
C.~Hadjivasiliou$^{6}$,
G.~Haefeli$^{45}$,
C.~Haen$^{44}$,
S.C.~Haines$^{51}$,
B.~Hamilton$^{62}$,
X.~Han$^{13}$,
T.H.~Hancock$^{59}$,
S.~Hansmann-Menzemer$^{13}$,
N.~Harnew$^{59}$,
T.~Harrison$^{56}$,
C.~Hasse$^{44}$,
M.~Hatch$^{44}$,
J.~He$^{66}$,
M.~Hecker$^{57}$,
K.~Heinicke$^{11}$,
A.~Heister$^{11}$,
K.~Hennessy$^{56}$,
L.~Henry$^{76}$,
E.~van~Herwijnen$^{44}$,
J.~Heuel$^{10}$,
M.~He{\ss}$^{71}$,
A.~Hicheur$^{64}$,
R.~Hidalgo~Charman$^{58}$,
D.~Hill$^{59}$,
M.~Hilton$^{58}$,
P.H.~Hopchev$^{45}$,
J.~Hu$^{13}$,
W.~Hu$^{69}$,
W.~Huang$^{66}$,
Z.C.~Huard$^{61}$,
W.~Hulsbergen$^{28}$,
T.~Humair$^{57}$,
M.~Hushchyn$^{39}$,
D.~Hutchcroft$^{56}$,
D.~Hynds$^{28}$,
P.~Ibis$^{11}$,
M.~Idzik$^{31}$,
P.~Ilten$^{49}$,
A.~Inglessi$^{34}$,
A.~Inyakin$^{41}$,
K.~Ivshin$^{34}$,
R.~Jacobsson$^{44}$,
J.~Jalocha$^{59}$,
E.~Jans$^{28}$,
B.K.~Jashal$^{76}$,
A.~Jawahery$^{62}$,
F.~Jiang$^{3}$,
M.~John$^{59}$,
D.~Johnson$^{44}$,
C.R.~Jones$^{51}$,
C.~Joram$^{44}$,
B.~Jost$^{44}$,
N.~Jurik$^{59}$,
S.~Kandybei$^{47}$,
M.~Karacson$^{44}$,
J.M.~Kariuki$^{50}$,
S.~Karodia$^{55}$,
N.~Kazeev$^{39}$,
M.~Kecke$^{13}$,
F.~Keizer$^{51}$,
M.~Kelsey$^{63}$,
M.~Kenzie$^{51}$,
T.~Ketel$^{29}$,
E.~Khairullin$^{38}$,
B.~Khanji$^{44}$,
C.~Khurewathanakul$^{45}$,
K.E.~Kim$^{63}$,
T.~Kirn$^{10}$,
V.S.~Kirsebom$^{45}$,
S.~Klaver$^{19}$,
K.~Klimaszewski$^{32}$,
T.~Klimkovich$^{12}$,
S.~Koliiev$^{48}$,
M.~Kolpin$^{13}$,
R.~Kopecna$^{13}$,
P.~Koppenburg$^{28}$,
I.~Kostiuk$^{28}$,
S.~Kotriakhova$^{34}$,
M.~Kozeiha$^{6}$,
L.~Kravchuk$^{37}$,
M.~Kreps$^{52}$,
F.~Kress$^{57}$,
P.~Krokovny$^{40,x}$,
W.~Krupa$^{31}$,
W.~Krzemien$^{32}$,
W.~Kucewicz$^{30,l}$,
M.~Kucharczyk$^{30}$,
V.~Kudryavtsev$^{40,x}$,
A.K.~Kuonen$^{45}$,
T.~Kvaratskheliya$^{35,44}$,
D.~Lacarrere$^{44}$,
G.~Lafferty$^{58}$,
A.~Lai$^{23}$,
D.~Lancierini$^{46}$,
G.~Lanfranchi$^{19}$,
C.~Langenbruch$^{10}$,
T.~Latham$^{52}$,
C.~Lazzeroni$^{49}$,
R.~Le~Gac$^{7}$,
A.~Leflat$^{36}$,
R.~Lef{\`e}vre$^{6}$,
F.~Lemaitre$^{44}$,
O.~Leroy$^{7}$,
T.~Lesiak$^{30}$,
B.~Leverington$^{13}$,
P.-R.~Li$^{66,ab}$,
Y.~Li$^{4}$,
Z.~Li$^{63}$,
X.~Liang$^{63}$,
T.~Likhomanenko$^{73}$,
R.~Lindner$^{44}$,
F.~Lionetto$^{46}$,
V.~Lisovskyi$^{8}$,
G.~Liu$^{67}$,
X.~Liu$^{3}$,
D.~Loh$^{52}$,
A.~Loi$^{23}$,
I.~Longstaff$^{55}$,
J.H.~Lopes$^{2}$,
G.H.~Lovell$^{51}$,
D.~Lucchesi$^{24,o}$,
M.~Lucio~Martinez$^{43}$,
A.~Lupato$^{24}$,
E.~Luppi$^{17,g}$,
O.~Lupton$^{44}$,
A.~Lusiani$^{25}$,
X.~Lyu$^{66}$,
F.~Machefert$^{8}$,
F.~Maciuc$^{33}$,
V.~Macko$^{45}$,
P.~Mackowiak$^{11}$,
S.~Maddrell-Mander$^{50}$,
O.~Maev$^{34,44}$,
K.~Maguire$^{58}$,
D.~Maisuzenko$^{34}$,
M.W.~Majewski$^{31}$,
S.~Malde$^{59}$,
B.~Malecki$^{44}$,
A.~Malinin$^{73}$,
T.~Maltsev$^{40,x}$,
G.~Manca$^{23,f}$,
G.~Mancinelli$^{7}$,
D.~Marangotto$^{22,q}$,
J.~Maratas$^{6,w}$,
J.F.~Marchand$^{5}$,
U.~Marconi$^{16}$,
C.~Marin~Benito$^{8}$,
M.~Marinangeli$^{45}$,
P.~Marino$^{45}$,
J.~Marks$^{13}$,
P.J.~Marshall$^{56}$,
G.~Martellotti$^{27}$,
M.~Martinelli$^{44}$,
D.~Martinez~Santos$^{43}$,
F.~Martinez~Vidal$^{76}$,
A.~Massafferri$^{1}$,
M.~Materok$^{10}$,
R.~Matev$^{44}$,
A.~Mathad$^{52}$,
Z.~Mathe$^{44}$,
C.~Matteuzzi$^{21}$,
A.~Mauri$^{46}$,
E.~Maurice$^{8,b}$,
B.~Maurin$^{45}$,
M.~McCann$^{57,44}$,
A.~McNab$^{58}$,
R.~McNulty$^{14}$,
J.V.~Mead$^{56}$,
B.~Meadows$^{61}$,
C.~Meaux$^{7}$,
N.~Meinert$^{71}$,
D.~Melnychuk$^{32}$,
M.~Merk$^{28}$,
A.~Merli$^{22,q}$,
E.~Michielin$^{24}$,
D.A.~Milanes$^{70}$,
E.~Millard$^{52}$,
M.-N.~Minard$^{5}$,
L.~Minzoni$^{17,g}$,
D.S.~Mitzel$^{13}$,
A.~Mogini$^{9}$,
R.D.~Moise$^{57}$,
T.~Momb{\"a}cher$^{11}$,
I.A.~Monroy$^{70}$,
S.~Monteil$^{6}$,
M.~Morandin$^{24}$,
G.~Morello$^{19}$,
M.J.~Morello$^{25,t}$,
O.~Morgunova$^{73}$,
J.~Moron$^{31}$,
A.B.~Morris$^{7}$,
R.~Mountain$^{63}$,
F.~Muheim$^{54}$,
M.~Mukherjee$^{69}$,
M.~Mulder$^{28}$,
C.H.~Murphy$^{59}$,
D.~Murray$^{58}$,
A.~M{\"o}dden~$^{11}$,
D.~M{\"u}ller$^{44}$,
J.~M{\"u}ller$^{11}$,
K.~M{\"u}ller$^{46}$,
V.~M{\"u}ller$^{11}$,
P.~Naik$^{50}$,
T.~Nakada$^{45}$,
R.~Nandakumar$^{53}$,
A.~Nandi$^{59}$,
T.~Nanut$^{45}$,
I.~Nasteva$^{2}$,
M.~Needham$^{54}$,
N.~Neri$^{22,q}$,
S.~Neubert$^{13}$,
N.~Neufeld$^{44}$,
R.~Newcombe$^{57}$,
T.D.~Nguyen$^{45}$,
C.~Nguyen-Mau$^{45,n}$,
S.~Nieswand$^{10}$,
R.~Niet$^{11}$,
N.~Nikitin$^{36}$,
A.~Nogay$^{73}$,
N.S.~Nolte$^{44}$,
D.P.~O'Hanlon$^{16}$,
A.~Oblakowska-Mucha$^{31}$,
V.~Obraztsov$^{41}$,
S.~Ogilvy$^{55}$,
R.~Oldeman$^{23,f}$,
C.J.G.~Onderwater$^{72}$,
A.~Ossowska$^{30}$,
J.M.~Otalora~Goicochea$^{2}$,
T.~Ovsiannikova$^{35}$,
P.~Owen$^{46}$,
A.~Oyanguren$^{76}$,
P.R.~Pais$^{45}$,
T.~Pajero$^{25,t}$,
A.~Palano$^{15}$,
M.~Palutan$^{19}$,
G.~Panshin$^{75}$,
A.~Papanestis$^{53}$,
M.~Pappagallo$^{54}$,
L.L.~Pappalardo$^{17,g}$,
W.~Parker$^{62}$,
C.~Parkes$^{58,44}$,
G.~Passaleva$^{18,44}$,
A.~Pastore$^{15}$,
M.~Patel$^{57}$,
C.~Patrignani$^{16,e}$,
A.~Pearce$^{44}$,
A.~Pellegrino$^{28}$,
G.~Penso$^{27}$,
M.~Pepe~Altarelli$^{44}$,
S.~Perazzini$^{44}$,
D.~Pereima$^{35}$,
P.~Perret$^{6}$,
L.~Pescatore$^{45}$,
K.~Petridis$^{50}$,
A.~Petrolini$^{20,h}$,
A.~Petrov$^{73}$,
S.~Petrucci$^{54}$,
M.~Petruzzo$^{22,q}$,
B.~Pietrzyk$^{5}$,
G.~Pietrzyk$^{45}$,
M.~Pikies$^{30}$,
M.~Pili$^{59}$,
D.~Pinci$^{27}$,
J.~Pinzino$^{44}$,
F.~Pisani$^{44}$,
A.~Piucci$^{13}$,
V.~Placinta$^{33}$,
S.~Playfer$^{54}$,
J.~Plews$^{49}$,
M.~Plo~Casasus$^{43}$,
F.~Polci$^{9}$,
M.~Poli~Lener$^{19}$,
A.~Poluektov$^{52}$,
N.~Polukhina$^{74,c}$,
I.~Polyakov$^{63}$,
E.~Polycarpo$^{2}$,
G.J.~Pomery$^{50}$,
S.~Ponce$^{44}$,
A.~Popov$^{41}$,
D.~Popov$^{49,12}$,
S.~Poslavskii$^{41}$,
E.~Price$^{50}$,
J.~Prisciandaro$^{43}$,
C.~Prouve$^{43}$,
V.~Pugatch$^{48}$,
A.~Puig~Navarro$^{46}$,
H.~Pullen$^{59}$,
G.~Punzi$^{25,p}$,
W.~Qian$^{66}$,
J.~Qin$^{66}$,
R.~Quagliani$^{9}$,
B.~Quintana$^{6}$,
N.V.~Raab$^{14}$,
B.~Rachwal$^{31}$,
J.H.~Rademacker$^{50}$,
M.~Rama$^{25}$,
M.~Ramos~Pernas$^{43}$,
M.S.~Rangel$^{2}$,
F.~Ratnikov$^{38,39}$,
G.~Raven$^{29}$,
M.~Ravonel~Salzgeber$^{44}$,
M.~Reboud$^{5}$,
F.~Redi$^{45}$,
S.~Reichert$^{11}$,
A.C.~dos~Reis$^{1}$,
F.~Reiss$^{9}$,
C.~Remon~Alepuz$^{76}$,
Z.~Ren$^{3}$,
V.~Renaudin$^{59}$,
S.~Ricciardi$^{53}$,
S.~Richards$^{50}$,
K.~Rinnert$^{56}$,
P.~Robbe$^{8}$,
A.~Robert$^{9}$,
A.B.~Rodrigues$^{45}$,
E.~Rodrigues$^{61}$,
J.A.~Rodriguez~Lopez$^{70}$,
M.~Roehrken$^{44}$,
S.~Roiser$^{44}$,
A.~Rollings$^{59}$,
V.~Romanovskiy$^{41}$,
A.~Romero~Vidal$^{43}$,
M.~Rotondo$^{19}$,
M.S.~Rudolph$^{63}$,
T.~Ruf$^{44}$,
J.~Ruiz~Vidal$^{76}$,
J.J.~Saborido~Silva$^{43}$,
N.~Sagidova$^{34}$,
B.~Saitta$^{23,f}$,
V.~Salustino~Guimaraes$^{65}$,
C.~Sanchez~Gras$^{28}$,
C.~Sanchez~Mayordomo$^{76}$,
B.~Sanmartin~Sedes$^{43}$,
R.~Santacesaria$^{27}$,
C.~Santamarina~Rios$^{43}$,
M.~Santimaria$^{19,44}$,
E.~Santovetti$^{26,j}$,
G.~Sarpis$^{58}$,
A.~Sarti$^{19,k}$,
C.~Satriano$^{27,s}$,
A.~Satta$^{26}$,
M.~Saur$^{66}$,
D.~Savrina$^{35,36}$,
S.~Schael$^{10}$,
M.~Schellenberg$^{11}$,
M.~Schiller$^{55}$,
H.~Schindler$^{44}$,
M.~Schmelling$^{12}$,
T.~Schmelzer$^{11}$,
B.~Schmidt$^{44}$,
O.~Schneider$^{45}$,
A.~Schopper$^{44}$,
H.F.~Schreiner$^{61}$,
M.~Schubiger$^{45}$,
S.~Schulte$^{45}$,
M.H.~Schune$^{8}$,
R.~Schwemmer$^{44}$,
B.~Sciascia$^{19}$,
A.~Sciubba$^{27,k}$,
A.~Semennikov$^{35}$,
E.S.~Sepulveda$^{9}$,
A.~Sergi$^{49}$,
N.~Serra$^{46}$,
J.~Serrano$^{7}$,
L.~Sestini$^{24}$,
A.~Seuthe$^{11}$,
P.~Seyfert$^{44}$,
M.~Shapkin$^{41}$,
Y.~Shcheglov$^{34,\dagger}$,
T.~Shears$^{56}$,
L.~Shekhtman$^{40,x}$,
V.~Shevchenko$^{73}$,
E.~Shmanin$^{74}$,
B.G.~Siddi$^{17}$,
R.~Silva~Coutinho$^{46}$,
L.~Silva~de~Oliveira$^{2}$,
G.~Simi$^{24,o}$,
S.~Simone$^{15,d}$,
I.~Skiba$^{17}$,
N.~Skidmore$^{13}$,
T.~Skwarnicki$^{63}$,
M.W.~Slater$^{49}$,
J.G.~Smeaton$^{51}$,
E.~Smith$^{10}$,
I.T.~Smith$^{54}$,
M.~Smith$^{57}$,
M.~Soares$^{16}$,
l.~Soares~Lavra$^{1}$,
M.D.~Sokoloff$^{61}$,
F.J.P.~Soler$^{55}$,
B.~Souza~De~Paula$^{2}$,
B.~Spaan$^{11}$,
E.~Spadaro~Norella$^{22,q}$,
P.~Spradlin$^{55}$,
F.~Stagni$^{44}$,
M.~Stahl$^{13}$,
S.~Stahl$^{44}$,
P.~Stefko$^{45}$,
S.~Stefkova$^{57}$,
O.~Steinkamp$^{46}$,
S.~Stemmle$^{13}$,
O.~Stenyakin$^{41}$,
M.~Stepanova$^{34}$,
H.~Stevens$^{11}$,
A.~Stocchi$^{8}$,
S.~Stone$^{63}$,
B.~Storaci$^{46}$,
S.~Stracka$^{25}$,
M.E.~Stramaglia$^{45}$,
M.~Straticiuc$^{33}$,
U.~Straumann$^{46}$,
S.~Strokov$^{75}$,
J.~Sun$^{3}$,
L.~Sun$^{68}$,
Y.~Sun$^{62}$,
K.~Swientek$^{31}$,
A.~Szabelski$^{32}$,
T.~Szumlak$^{31}$,
M.~Szymanski$^{66}$,
S.~T'Jampens$^{5}$,
Z.~Tang$^{3}$,
A.~Tayduganov$^{7}$,
T.~Tekampe$^{11}$,
G.~Tellarini$^{17}$,
F.~Teubert$^{44}$,
E.~Thomas$^{44}$,
J.~van~Tilburg$^{28}$,
M.J.~Tilley$^{57}$,
V.~Tisserand$^{6}$,
M.~Tobin$^{31}$,
S.~Tolk$^{44}$,
L.~Tomassetti$^{17,g}$,
D.~Tonelli$^{25}$,
D.Y.~Tou$^{9}$,
R.~Tourinho~Jadallah~Aoude$^{1}$,
E.~Tournefier$^{5}$,
M.~Traill$^{55}$,
M.T.~Tran$^{45}$,
A.~Trisovic$^{51}$,
A.~Tsaregorodtsev$^{7}$,
G.~Tuci$^{25,p}$,
A.~Tully$^{51}$,
N.~Tuning$^{28,44}$,
A.~Ukleja$^{32}$,
A.~Usachov$^{8}$,
A.~Ustyuzhanin$^{38,39}$,
U.~Uwer$^{13}$,
A.~Vagner$^{75}$,
V.~Vagnoni$^{16}$,
A.~Valassi$^{44}$,
S.~Valat$^{44}$,
G.~Valenti$^{16}$,
R.~Vazquez~Gomez$^{44}$,
P.~Vazquez~Regueiro$^{43}$,
S.~Vecchi$^{17}$,
M.~van~Veghel$^{28}$,
J.J.~Velthuis$^{50}$,
M.~Veltri$^{18,r}$,
G.~Veneziano$^{59}$,
A.~Venkateswaran$^{63}$,
M.~Vernet$^{6}$,
M.~Veronesi$^{28}$,
M.~Vesterinen$^{52}$,
J.V.~Viana~Barbosa$^{44}$,
D.~~Vieira$^{66}$,
M.~Vieites~Diaz$^{43}$,
H.~Viemann$^{71}$,
X.~Vilasis-Cardona$^{42,m}$,
A.~Vitkovskiy$^{28}$,
M.~Vitti$^{51}$,
V.~Volkov$^{36}$,
A.~Vollhardt$^{46}$,
D.~Vom~Bruch$^{9}$,
B.~Voneki$^{44}$,
A.~Vorobyev$^{34}$,
V.~Vorobyev$^{40,x}$,
N.~Voropaev$^{34}$,
J.A.~de~Vries$^{28}$,
C.~V{\'a}zquez~Sierra$^{28}$,
R.~Waldi$^{71}$,
J.~Walsh$^{25}$,
J.~Wang$^{4}$,
M.~Wang$^{3}$,
Y.~Wang$^{69}$,
Z.~Wang$^{46}$,
D.R.~Ward$^{51}$,
H.M.~Wark$^{56}$,
N.K.~Watson$^{49}$,
D.~Websdale$^{57}$,
A.~Weiden$^{46}$,
C.~Weisser$^{60}$,
M.~Whitehead$^{10}$,
G.~Wilkinson$^{59}$,
M.~Wilkinson$^{63}$,
I.~Williams$^{51}$,
M.R.J.~Williams$^{58}$,
M.~Williams$^{60}$,
T.~Williams$^{49}$,
F.F.~Wilson$^{53}$,
M.~Winn$^{8}$,
W.~Wislicki$^{32}$,
M.~Witek$^{30}$,
G.~Wormser$^{8}$,
S.A.~Wotton$^{51}$,
K.~Wyllie$^{44}$,
D.~Xiao$^{69}$,
Y.~Xie$^{69}$,
A.~Xu$^{3}$,
M.~Xu$^{69}$,
Q.~Xu$^{66}$,
Z.~Xu$^{3}$,
Z.~Xu$^{5}$,
Z.~Yang$^{3}$,
Z.~Yang$^{62}$,
Y.~Yao$^{63}$,
L.E.~Yeomans$^{56}$,
H.~Yin$^{69}$,
J.~Yu$^{69,aa}$,
X.~Yuan$^{63}$,
O.~Yushchenko$^{41}$,
K.A.~Zarebski$^{49}$,
M.~Zavertyaev$^{12,c}$,
D.~Zhang$^{69}$,
L.~Zhang$^{3}$,
W.C.~Zhang$^{3,z}$,
Y.~Zhang$^{44}$,
A.~Zhelezov$^{13}$,
Y.~Zheng$^{66}$,
X.~Zhu$^{3}$,
V.~Zhukov$^{10,36}$,
J.B.~Zonneveld$^{54}$,
S.~Zucchelli$^{16}$.\bigskip

{\footnotesize \it
$ ^{1}$Centro Brasileiro de Pesquisas F{\'\i}sicas (CBPF), Rio de Janeiro, Brazil\\
$ ^{2}$Universidade Federal do Rio de Janeiro (UFRJ), Rio de Janeiro, Brazil\\
$ ^{3}$Center for High Energy Physics, Tsinghua University, Beijing, China\\
$ ^{4}$Institute Of High Energy Physics (ihep), Beijing, China\\
$ ^{5}$Univ. Grenoble Alpes, Univ. Savoie Mont Blanc, CNRS, IN2P3-LAPP, Annecy, France\\
$ ^{6}$Universit{\'e} Clermont Auvergne, CNRS/IN2P3, LPC, Clermont-Ferrand, France\\
$ ^{7}$Aix Marseille Univ, CNRS/IN2P3, CPPM, Marseille, France\\
$ ^{8}$LAL, Univ. Paris-Sud, CNRS/IN2P3, Universit{\'e} Paris-Saclay, Orsay, France\\
$ ^{9}$LPNHE, Sorbonne Universit{\'e}, Paris Diderot Sorbonne Paris Cit{\'e}, CNRS/IN2P3, Paris, France\\
$ ^{10}$I. Physikalisches Institut, RWTH Aachen University, Aachen, Germany\\
$ ^{11}$Fakult{\"a}t Physik, Technische Universit{\"a}t Dortmund, Dortmund, Germany\\
$ ^{12}$Max-Planck-Institut f{\"u}r Kernphysik (MPIK), Heidelberg, Germany\\
$ ^{13}$Physikalisches Institut, Ruprecht-Karls-Universit{\"a}t Heidelberg, Heidelberg, Germany\\
$ ^{14}$School of Physics, University College Dublin, Dublin, Ireland\\
$ ^{15}$INFN Sezione di Bari, Bari, Italy\\
$ ^{16}$INFN Sezione di Bologna, Bologna, Italy\\
$ ^{17}$INFN Sezione di Ferrara, Ferrara, Italy\\
$ ^{18}$INFN Sezione di Firenze, Firenze, Italy\\
$ ^{19}$INFN Laboratori Nazionali di Frascati, Frascati, Italy\\
$ ^{20}$INFN Sezione di Genova, Genova, Italy\\
$ ^{21}$INFN Sezione di Milano-Bicocca, Milano, Italy\\
$ ^{22}$INFN Sezione di Milano, Milano, Italy\\
$ ^{23}$INFN Sezione di Cagliari, Monserrato, Italy\\
$ ^{24}$INFN Sezione di Padova, Padova, Italy\\
$ ^{25}$INFN Sezione di Pisa, Pisa, Italy\\
$ ^{26}$INFN Sezione di Roma Tor Vergata, Roma, Italy\\
$ ^{27}$INFN Sezione di Roma La Sapienza, Roma, Italy\\
$ ^{28}$Nikhef National Institute for Subatomic Physics, Amsterdam, Netherlands\\
$ ^{29}$Nikhef National Institute for Subatomic Physics and VU University Amsterdam, Amsterdam, Netherlands\\
$ ^{30}$Henryk Niewodniczanski Institute of Nuclear Physics  Polish Academy of Sciences, Krak{\'o}w, Poland\\
$ ^{31}$AGH - University of Science and Technology, Faculty of Physics and Applied Computer Science, Krak{\'o}w, Poland\\
$ ^{32}$National Center for Nuclear Research (NCBJ), Warsaw, Poland\\
$ ^{33}$Horia Hulubei National Institute of Physics and Nuclear Engineering, Bucharest-Magurele, Romania\\
$ ^{34}$Petersburg Nuclear Physics Institute (PNPI), Gatchina, Russia\\
$ ^{35}$Institute of Theoretical and Experimental Physics (ITEP), Moscow, Russia\\
$ ^{36}$Institute of Nuclear Physics, Moscow State University (SINP MSU), Moscow, Russia\\
$ ^{37}$Institute for Nuclear Research of the Russian Academy of Sciences (INR RAS), Moscow, Russia\\
$ ^{38}$Yandex School of Data Analysis, Moscow, Russia\\
$ ^{39}$National Research University Higher School of Economics, Moscow, Russia\\
$ ^{40}$Budker Institute of Nuclear Physics (SB RAS), Novosibirsk, Russia\\
$ ^{41}$Institute for High Energy Physics (IHEP), Protvino, Russia\\
$ ^{42}$ICCUB, Universitat de Barcelona, Barcelona, Spain\\
$ ^{43}$Instituto Galego de F{\'\i}sica de Altas Enerx{\'\i}as (IGFAE), Universidade de Santiago de Compostela, Santiago de Compostela, Spain\\
$ ^{44}$European Organization for Nuclear Research (CERN), Geneva, Switzerland\\
$ ^{45}$Institute of Physics, Ecole Polytechnique  F{\'e}d{\'e}rale de Lausanne (EPFL), Lausanne, Switzerland\\
$ ^{46}$Physik-Institut, Universit{\"a}t Z{\"u}rich, Z{\"u}rich, Switzerland\\
$ ^{47}$NSC Kharkiv Institute of Physics and Technology (NSC KIPT), Kharkiv, Ukraine\\
$ ^{48}$Institute for Nuclear Research of the National Academy of Sciences (KINR), Kyiv, Ukraine\\
$ ^{49}$University of Birmingham, Birmingham, United Kingdom\\
$ ^{50}$H.H. Wills Physics Laboratory, University of Bristol, Bristol, United Kingdom\\
$ ^{51}$Cavendish Laboratory, University of Cambridge, Cambridge, United Kingdom\\
$ ^{52}$Department of Physics, University of Warwick, Coventry, United Kingdom\\
$ ^{53}$STFC Rutherford Appleton Laboratory, Didcot, United Kingdom\\
$ ^{54}$School of Physics and Astronomy, University of Edinburgh, Edinburgh, United Kingdom\\
$ ^{55}$School of Physics and Astronomy, University of Glasgow, Glasgow, United Kingdom\\
$ ^{56}$Oliver Lodge Laboratory, University of Liverpool, Liverpool, United Kingdom\\
$ ^{57}$Imperial College London, London, United Kingdom\\
$ ^{58}$School of Physics and Astronomy, University of Manchester, Manchester, United Kingdom\\
$ ^{59}$Department of Physics, University of Oxford, Oxford, United Kingdom\\
$ ^{60}$Massachusetts Institute of Technology, Cambridge, MA, United States\\
$ ^{61}$University of Cincinnati, Cincinnati, OH, United States\\
$ ^{62}$University of Maryland, College Park, MD, United States\\
$ ^{63}$Syracuse University, Syracuse, NY, United States\\
$ ^{64}$Laboratory of Mathematical and Subatomic Physics , Constantine, Algeria, associated to $^{2}$\\
$ ^{65}$Pontif{\'\i}cia Universidade Cat{\'o}lica do Rio de Janeiro (PUC-Rio), Rio de Janeiro, Brazil, associated to $^{2}$\\
$ ^{66}$University of Chinese Academy of Sciences, Beijing, China, associated to $^{3}$\\
$ ^{67}$South China Normal University, Guangzhou, China, associated to $^{3}$\\
$ ^{68}$School of Physics and Technology, Wuhan University, Wuhan, China, associated to $^{3}$\\
$ ^{69}$Institute of Particle Physics, Central China Normal University, Wuhan, Hubei, China, associated to $^{3}$\\
$ ^{70}$Departamento de Fisica , Universidad Nacional de Colombia, Bogota, Colombia, associated to $^{9}$\\
$ ^{71}$Institut f{\"u}r Physik, Universit{\"a}t Rostock, Rostock, Germany, associated to $^{13}$\\
$ ^{72}$Van Swinderen Institute, University of Groningen, Groningen, Netherlands, associated to $^{28}$\\
$ ^{73}$National Research Centre Kurchatov Institute, Moscow, Russia, associated to $^{35}$\\
$ ^{74}$National University of Science and Technology ``MISIS'', Moscow, Russia, associated to $^{35}$\\
$ ^{75}$National Research Tomsk Polytechnic University, Tomsk, Russia, associated to $^{35}$\\
$ ^{76}$Instituto de Fisica Corpuscular, Centro Mixto Universidad de Valencia - CSIC, Valencia, Spain, associated to $^{42}$\\
$ ^{77}$H.H. Wills Physics Laboratory, University of Bristol, Bristol, United Kingdom, Bristol, United Kingdom\\
$ ^{78}$University of Michigan, Ann Arbor, United States, associated to $^{63}$\\
$ ^{79}$Los Alamos National Laboratory (LANL), Los Alamos, United States, associated to $^{63}$\\
\bigskip
$ ^{a}$Universidade Federal do Tri{\^a}ngulo Mineiro (UFTM), Uberaba-MG, Brazil\\
$ ^{b}$Laboratoire Leprince-Ringuet, Palaiseau, France\\
$ ^{c}$P.N. Lebedev Physical Institute, Russian Academy of Science (LPI RAS), Moscow, Russia\\
$ ^{d}$Universit{\`a} di Bari, Bari, Italy\\
$ ^{e}$Universit{\`a} di Bologna, Bologna, Italy\\
$ ^{f}$Universit{\`a} di Cagliari, Cagliari, Italy\\
$ ^{g}$Universit{\`a} di Ferrara, Ferrara, Italy\\
$ ^{h}$Universit{\`a} di Genova, Genova, Italy\\
$ ^{i}$Universit{\`a} di Milano Bicocca, Milano, Italy\\
$ ^{j}$Universit{\`a} di Roma Tor Vergata, Roma, Italy\\
$ ^{k}$Universit{\`a} di Roma La Sapienza, Roma, Italy\\
$ ^{l}$AGH - University of Science and Technology, Faculty of Computer Science, Electronics and Telecommunications, Krak{\'o}w, Poland\\
$ ^{m}$LIFAELS, La Salle, Universitat Ramon Llull, Barcelona, Spain\\
$ ^{n}$Hanoi University of Science, Hanoi, Vietnam\\
$ ^{o}$Universit{\`a} di Padova, Padova, Italy\\
$ ^{p}$Universit{\`a} di Pisa, Pisa, Italy\\
$ ^{q}$Universit{\`a} degli Studi di Milano, Milano, Italy\\
$ ^{r}$Universit{\`a} di Urbino, Urbino, Italy\\
$ ^{s}$Universit{\`a} della Basilicata, Potenza, Italy\\
$ ^{t}$Scuola Normale Superiore, Pisa, Italy\\
$ ^{u}$Universit{\`a} di Modena e Reggio Emilia, Modena, Italy\\
$ ^{v}$H.H. Wills Physics Laboratory, University of Bristol, Bristol, United Kingdom\\
$ ^{w}$MSU - Iligan Institute of Technology (MSU-IIT), Iligan, Philippines\\
$ ^{x}$Novosibirsk State University, Novosibirsk, Russia\\
$ ^{y}$Sezione INFN di Trieste, Trieste, Italy\\
$ ^{z}$School of Physics and Information Technology, Shaanxi Normal University (SNNU), Xi'an, China\\
$ ^{aa}$Physics and Micro Electronic College, Hunan University, Changsha City, China\\
$ ^{ab}$Lanzhou University, Lanzhou, China\\
\medskip
$ ^{\dagger}$Deceased
}
\end{flushleft}

==> LHCb_Authorship_flat_arXiv_02-Oct-2018.tex <==
LHCb collaboration: 
R. Aaij,
C. Abell{\'a}n Beteta,
B. Adeva,
M. Adinolfi,
C.A. Aidala,
Z. Ajaltouni,
S. Akar,
P. Albicocco,
J. Albrecht,
F. Alessio,
M. Alexander,
A. Alfonso Albero,
G. Alkhazov,
P. Alvarez Cartelle,
A.A. Alves Jr,
S. Amato,
S. Amerio,
Y. Amhis,
L. An,
L. Anderlini,
G. Andreassi,
M. Andreotti,
J.E. Andrews,
F. Archilli,
P. d'Argent,
J. Arnau Romeu,
A. Artamonov,
M. Artuso,
K. Arzymatov,
E. Aslanides,
M. Atzeni,
B. Audurier,
S. Bachmann,
J.J. Back,
S. Baker,
V. Balagura,
W. Baldini,
A. Baranov,
R.J. Barlow,
G.C. Barrand,
S. Barsuk,
W. Barter,
M. Bartolini,
F. Baryshnikov,
V. Batozskaya,
B. Batsukh,
A. Battig,
V. Battista,
A. Bay,
J. Beddow,
F. Bedeschi,
I. Bediaga,
A. Beiter,
L.J. Bel,
S. Belin,
N. Beliy,
V. Bellee,
N. Belloli,
K. Belous,
I. Belyaev,
E. Ben-Haim,
G. Bencivenni,
S. Benson,
S. Beranek,
A. Berezhnoy,
R. Bernet,
D. Berninghoff,
E. Bertholet,
A. Bertolin,
C. Betancourt,
F. Betti,
M.O. Bettler,
M. van Beuzekom,
Ia. Bezshyiko,
S. Bhasin,
J. Bhom,
S. Bifani,
P. Billoir,
A. Birnkraut,
A. Bizzeti,
M. Bj{\o}rn,
M.P. Blago,
T. Blake,
F. Blanc,
S. Blusk,
D. Bobulska,
V. Bocci,
O. Boente Garcia,
T. Boettcher,
A. Bondar,
N. Bondar,
S. Borghi,
M. Borisyak,
M. Borsato,
F. Bossu,
M. Boubdir,
T.J.V. Bowcock,
C. Bozzi,
S. Braun,
M. Brodski,
J. Brodzicka,
A. Brossa Gonzalo,
D. Brundu,
E. Buchanan,
A. Buonaura,
C. Burr,
A. Bursche,
J. Buytaert,
W. Byczynski,
S. Cadeddu,
H. Cai,
R. Calabrese,
R. Calladine,
M. Calvi,
M. Calvo Gomez,
A. Camboni,
P. Campana,
D.H. Campora Perez,
L. Capriotti,
A. Carbone,
G. Carboni,
R. Cardinale,
A. Cardini,
P. Carniti,
K. Carvalho Akiba,
G. Casse,
L. Cassina,
M. Cattaneo,
G. Cavallero,
R. Cenci,
D. Chamont,
M.G. Chapman,
M. Charles,
Ph. Charpentier,
G. Chatzikonstantinidis,
M. Chefdeville,
V. Chekalina,
C. Chen,
S. Chen,
S.-G. Chitic,
V. Chobanova,
M. Chrzaszcz,
A. Chubykin,
P. Ciambrone,
X. Cid Vidal,
G. Ciezarek,
F. Cindolo,
P.E.L. Clarke,
M. Clemencic,
H.V. Cliff,
J. Closier,
V. Coco,
J.A.B. Coelho,
J. Cogan,
E. Cogneras,
L. Cojocariu,
P. Collins,
T. Colombo,
A. Comerma-Montells,
A. Contu,
G. Coombs,
S. Coquereau,
G. Corti,
M. Corvo,
C.M. Costa Sobral,
B. Couturier,
G.A. Cowan,
D.C. Craik,
A. Crocombe,
M. Cruz Torres,
R. Currie,
C. D'Ambrosio,
F. Da Cunha Marinho,
C.L. Da Silva,
E. Dall'Occo,
J. Dalseno,
A. Danilina,
A. Davis,
O. De Aguiar Francisco,
K. De Bruyn,
S. De Capua,
M. De Cian,
J.M. De Miranda,
L. De Paula,
M. De Serio,
P. De Simone,
C.T. Dean,
D. Decamp,
L. Del Buono,
B. Delaney,
H.-P. Dembinski,
M. Demmer,
A. Dendek,
D. Derkach,
O. Deschamps,
F. Desse,
F. Dettori,
B. Dey,
A. Di Canto,
P. Di Nezza,
S. Didenko,
H. Dijkstra,
F. Dordei,
M. Dorigo,
A. Dosil Su{\'a}rez,
L. Douglas,
A. Dovbnya,
K. Dreimanis,
L. Dufour,
G. Dujany,
P. Durante,
J.M. Durham,
D. Dutta,
R. Dzhelyadin,
M. Dziewiecki,
A. Dziurda,
A. Dzyuba,
S. Easo,
U. Egede,
V. Egorychev,
S. Eidelman,
S. Eisenhardt,
U. Eitschberger,
R. Ekelhof,
L. Eklund,
S. Ely,
A. Ene,
S. Escher,
S. Esen,
T. Evans,
A. Falabella,
N. Farley,
S. Farry,
D. Fazzini,
P. Fernandez Declara,
A. Fernandez Prieto,
F. Ferrari,
L. Ferreira Lopes,
F. Ferreira Rodrigues,
M. Ferro-Luzzi,
S. Filippov,
R.A. Fini,
M. Fiorini,
M. Firlej,
C. Fitzpatrick,
T. Fiutowski,
F. Fleuret,
M. Fontana,
F. Fontanelli,
R. Forty,
V. Franco Lima,
M. Frank,
C. Frei,
J. Fu,
W. Funk,
C. F{\"a}rber,
M. F{\'e}o,
E. Gabriel,
A. Gallas Torreira,
D. Galli,
S. Gallorini,
S. Gambetta,
Y. Gan,
M. Gandelman,
P. Gandini,
Y. Gao,
L.M. Garcia Martin,
B. Garcia Plana,
J. Garc{\'\i}a Pardi{\~n}as,
J. Garra Tico,
L. Garrido,
D. Gascon,
C. Gaspar,
L. Gavardi,
G. Gazzoni,
D. Gerick,
E. Gersabeck,
M. Gersabeck,
T. Gershon,
D. Gerstel,
Ph. Ghez,
V. Gibson,
O.G. Girard,
P. Gironella Gironell,
L. Giubega,
K. Gizdov,
V.V. Gligorov,
D. Golubkov,
A. Golutvin,
A. Gomes,
I.V. Gorelov,
C. Gotti,
E. Govorkova,
J.P. Grabowski,
R. Graciani Diaz,
L.A. Granado Cardoso,
E. Graug{\'e}s,
E. Graverini,
G. Graziani,
A. Grecu,
R. Greim,
P. Griffith,
L. Grillo,
L. Gruber,
B.R. Gruberg Cazon,
O. Gr{\"u}nberg,
C. Gu,
E. Gushchin,
A. Guth,
Yu. Guz,
T. Gys,
C. G{\"o}bel,
T. Hadavizadeh,
C. Hadjivasiliou,
G. Haefeli,
C. Haen,
S.C. Haines,
B. Hamilton,
X. Han,
T.H. Hancock,
S. Hansmann-Menzemer,
N. Harnew,
T. Harrison,
C. Hasse,
M. Hatch,
J. He,
M. Hecker,
K. Heinicke,
A. Heister,
K. Hennessy,
L. Henry,
E. van Herwijnen,
J. Heuel,
M. He{\ss},
A. Hicheur,
R. Hidalgo Charman,
D. Hill,
M. Hilton,
P.H. Hopchev,
J. Hu,
W. Hu,
W. Huang,
Z.C. Huard,
W. Hulsbergen,
T. Humair,
M. Hushchyn,
D. Hutchcroft,
D. Hynds,
P. Ibis,
M. Idzik,
P. Ilten,
A. Inglessi,
A. Inyakin,
K. Ivshin,
R. Jacobsson,
J. Jalocha,
E. Jans,
B.K. Jashal,
A. Jawahery,
F. Jiang,
M. John,
D. Johnson,
C.R. Jones,
C. Joram,
B. Jost,
N. Jurik,
S. Kandybei,
M. Karacson,
J.M. Kariuki,
S. Karodia,
N. Kazeev,
M. Kecke,
F. Keizer,
M. Kelsey,
M. Kenzie,
T. Ketel,
E. Khairullin,
B. Khanji,
C. Khurewathanakul,
K.E. Kim,
T. Kirn,
V.S. Kirsebom,
S. Klaver,
K. Klimaszewski,
T. Klimkovich,
S. Koliiev,
M. Kolpin,
R. Kopecna,
P. Koppenburg,
I. Kostiuk,
S. Kotriakhova,
M. Kozeiha,
L. Kravchuk,
M. Kreps,
F. Kress,
P. Krokovny,
W. Krupa,
W. Krzemien,
W. Kucewicz,
M. Kucharczyk,
V. Kudryavtsev,
A.K. Kuonen,
T. Kvaratskheliya,
D. Lacarrere,
G. Lafferty,
A. Lai,
D. Lancierini,
G. Lanfranchi,
C. Langenbruch,
T. Latham,
C. Lazzeroni,
R. Le Gac,
A. Leflat,
R. Lef{\`e}vre,
F. Lemaitre,
O. Leroy,
T. Lesiak,
B. Leverington,
P.-R. Li,
Y. Li,
Z. Li,
X. Liang,
T. Likhomanenko,
R. Lindner,
F. Lionetto,
V. Lisovskyi,
G. Liu,
X. Liu,
D. Loh,
A. Loi,
I. Longstaff,
J.H. Lopes,
G.H. Lovell,
D. Lucchesi,
M. Lucio Martinez,
A. Lupato,
E. Luppi,
O. Lupton,
A. Lusiani,
X. Lyu,
F. Machefert,
F. Maciuc,
V. Macko,
P. Mackowiak,
S. Maddrell-Mander,
O. Maev,
K. Maguire,
D. Maisuzenko,
M.W. Majewski,
S. Malde,
B. Malecki,
A. Malinin,
T. Maltsev,
G. Manca,
G. Mancinelli,
D. Marangotto,
J. Maratas,
J.F. Marchand,
U. Marconi,
C. Marin Benito,
M. Marinangeli,
P. Marino,
J. Marks,
P.J. Marshall,
G. Martellotti,
M. Martinelli,
D. Martinez Santos,
F. Martinez Vidal,
A. Massafferri,
M. Materok,
R. Matev,
A. Mathad,
Z. Mathe,
C. Matteuzzi,
A. Mauri,
E. Maurice,
B. Maurin,
M. McCann,
A. McNab,
R. McNulty,
J.V. Mead,
B. Meadows,
C. Meaux,
N. Meinert,
D. Melnychuk,
M. Merk,
A. Merli,
E. Michielin,
D.A. Milanes,
E. Millard,
M.-N. Minard,
L. Minzoni,
D.S. Mitzel,
A. Mogini,
R.D. Moise,
T. Momb{\"a}cher,
I.A. Monroy,
S. Monteil,
M. Morandin,
G. Morello,
M.J. Morello,
O. Morgunova,
J. Moron,
A.B. Morris,
R. Mountain,
F. Muheim,
M. Mukherjee,
M. Mulder,
C.H. Murphy,
D. Murray,
A. M{\"o}dden ,
D. M{\"u}ller,
J. M{\"u}ller,
K. M{\"u}ller,
V. M{\"u}ller,
P. Naik,
T. Nakada,
R. Nandakumar,
A. Nandi,
T. Nanut,
I. Nasteva,
M. Needham,
N. Neri,
S. Neubert,
N. Neufeld,
R. Newcombe,
T.D. Nguyen,
C. Nguyen-Mau,
S. Nieswand,
R. Niet,
N. Nikitin,
A. Nogay,
N.S. Nolte,
D.P. O'Hanlon,
A. Oblakowska-Mucha,
V. Obraztsov,
S. Ogilvy,
R. Oldeman,
C.J.G. Onderwater,
A. Ossowska,
J.M. Otalora Goicochea,
T. Ovsiannikova,
P. Owen,
A. Oyanguren,
P.R. Pais,
T. Pajero,
A. Palano,
M. Palutan,
G. Panshin,
A. Papanestis,
M. Pappagallo,
L.L. Pappalardo,
W. Parker,
C. Parkes,
G. Passaleva,
A. Pastore,
M. Patel,
C. Patrignani,
A. Pearce,
A. Pellegrino,
G. Penso,
M. Pepe Altarelli,
S. Perazzini,
D. Pereima,
P. Perret,
L. Pescatore,
K. Petridis,
A. Petrolini,
A. Petrov,
S. Petrucci,
M. Petruzzo,
B. Pietrzyk,
G. Pietrzyk,
M. Pikies,
M. Pili,
D. Pinci,
J. Pinzino,
F. Pisani,
A. Piucci,
V. Placinta,
S. Playfer,
J. Plews,
M. Plo Casasus,
F. Polci,
M. Poli Lener,
A. Poluektov,
N. Polukhina,
I. Polyakov,
E. Polycarpo,
G.J. Pomery,
S. Ponce,
A. Popov,
D. Popov,
S. Poslavskii,
E. Price,
J. Prisciandaro,
C. Prouve,
V. Pugatch,
A. Puig Navarro,
H. Pullen,
G. Punzi,
W. Qian,
J. Qin,
R. Quagliani,
B. Quintana,
N.V. Raab,
B. Rachwal,
J.H. Rademacker,
M. Rama,
M. Ramos Pernas,
M.S. Rangel,
F. Ratnikov,
G. Raven,
M. Ravonel Salzgeber,
M. Reboud,
F. Redi,
S. Reichert,
A.C. dos Reis,
F. Reiss,
C. Remon Alepuz,
Z. Ren,
V. Renaudin,
S. Ricciardi,
S. Richards,
K. Rinnert,
P. Robbe,
A. Robert,
A.B. Rodrigues,
E. Rodrigues,
J.A. Rodriguez Lopez,
M. Roehrken,
S. Roiser,
A. Rollings,
V. Romanovskiy,
A. Romero Vidal,
M. Rotondo,
M.S. Rudolph,
T. Ruf,
J. Ruiz Vidal,
J.J. Saborido Silva,
N. Sagidova,
B. Saitta,
V. Salustino Guimaraes,
C. Sanchez Gras,
C. Sanchez Mayordomo,
B. Sanmartin Sedes,
R. Santacesaria,
C. Santamarina Rios,
M. Santimaria,
E. Santovetti,
G. Sarpis,
A. Sarti,
C. Satriano,
A. Satta,
M. Saur,
D. Savrina,
S. Schael,
M. Schellenberg,
M. Schiller,
H. Schindler,
M. Schmelling,
T. Schmelzer,
B. Schmidt,
O. Schneider,
A. Schopper,
H.F. Schreiner,
M. Schubiger,
S. Schulte,
M.H. Schune,
R. Schwemmer,
B. Sciascia,
A. Sciubba,
A. Semennikov,
E.S. Sepulveda,
A. Sergi,
N. Serra,
J. Serrano,
L. Sestini,
A. Seuthe,
P. Seyfert,
M. Shapkin,
Y. Shcheglov,
T. Shears,
L. Shekhtman,
V. Shevchenko,
E. Shmanin,
B.G. Siddi,
R. Silva Coutinho,
L. Silva de Oliveira,
G. Simi,
S. Simone,
I. Skiba,
N. Skidmore,
T. Skwarnicki,
M.W. Slater,
J.G. Smeaton,
E. Smith,
I.T. Smith,
M. Smith,
M. Soares,
l. Soares Lavra,
M.D. Sokoloff,
F.J.P. Soler,
B. Souza De Paula,
B. Spaan,
E. Spadaro Norella,
P. Spradlin,
F. Stagni,
M. Stahl,
S. Stahl,
P. Stefko,
S. Stefkova,
O. Steinkamp,
S. Stemmle,
O. Stenyakin,
M. Stepanova,
H. Stevens,
A. Stocchi,
S. Stone,
B. Storaci,
S. Stracka,
M.E. Stramaglia,
M. Straticiuc,
U. Straumann,
S. Strokov,
J. Sun,
L. Sun,
Y. Sun,
K. Swientek,
A. Szabelski,
T. Szumlak,
M. Szymanski,
S. T'Jampens,
Z. Tang,
A. Tayduganov,
T. Tekampe,
G. Tellarini,
F. Teubert,
E. Thomas,
J. van Tilburg,
M.J. Tilley,
V. Tisserand,
M. Tobin,
S. Tolk,
L. Tomassetti,
D. Tonelli,
D.Y. Tou,
R. Tourinho Jadallah Aoude,
E. Tournefier,
M. Traill,
M.T. Tran,
A. Trisovic,
A. Tsaregorodtsev,
G. Tuci,
A. Tully,
N. Tuning,
A. Ukleja,
A. Usachov,
A. Ustyuzhanin,
U. Uwer,
A. Vagner,
V. Vagnoni,
A. Valassi,
S. Valat,
G. Valenti,
R. Vazquez Gomez,
P. Vazquez Regueiro,
S. Vecchi,
M. van Veghel,
J.J. Velthuis,
M. Veltri,
G. Veneziano,
A. Venkateswaran,
M. Vernet,
M. Veronesi,
M. Vesterinen,
J.V. Viana Barbosa,
D.  Vieira,
M. Vieites Diaz,
H. Viemann,
X. Vilasis-Cardona,
A. Vitkovskiy,
M. Vitti,
V. Volkov,
A. Vollhardt,
D. Vom Bruch,
B. Voneki,
A. Vorobyev,
V. Vorobyev,
N. Voropaev,
J.A. de Vries,
C. V{\'a}zquez Sierra,
R. Waldi,
J. Walsh,
J. Wang,
M. Wang,
Y. Wang,
Z. Wang,
D.R. Ward,
H.M. Wark,
N.K. Watson,
D. Websdale,
A. Weiden,
C. Weisser,
M. Whitehead,
G. Wilkinson,
M. Wilkinson,
I. Williams,
M.R.J. Williams,
M. Williams,
T. Williams,
F.F. Wilson,
M. Winn,
W. Wislicki,
M. Witek,
G. Wormser,
S.A. Wotton,
K. Wyllie,
D. Xiao,
Y. Xie,
A. Xu,
M. Xu,
Q. Xu,
Z. Xu,
Z. Xu,
Z. Yang,
Z. Yang,
Y. Yao,
L.E. Yeomans,
H. Yin,
J. Yu,
X. Yuan,
O. Yushchenko,
K.A. Zarebski,
M. Zavertyaev,
D. Zhang,
L. Zhang,
W.C. Zhang,
Y. Zhang,
A. Zhelezov,
Y. Zheng,
X. Zhu,
V. Zhukov,
J.B. Zonneveld,
S. Zucchelli

==> LHCb_authorlist.tex <==
% $Id: LHCb_authorlist.tex 78711 2015-08-06 07:54:32Z apuignav $
% ===============================================================================
% Purpose: example of authorlist for LHCb template
% Author:
% Created on: 2009-09-24
% ===============================================================================

%\documentclass[a4paper]{article}
%\setlength{\oddsidemargin}{0cm}
%\setlength{\evensidemargin}{0cm}
%\setlength{\textwidth}{16.5cm}
%\setlength{\parindent}{0cm}
%\begin{document}
\centerline{\large\normalfont\bfseries LHCb collaboration}
\begin{flushleft}
\small
%-- LHCb Authorlist, Example typesetting
%-- 
A.~N.~Other$^{1}$.\bigskip\newline{\it
\footnotesize
$ ^{1}$University of nowhere\\
}
%-- 
%-- 
\end{flushleft}
%\end{document}


==> Makefile <==
# $Id: Makefile 119978 2018-05-08 14:31:46Z pkoppenb $
# ===============================================================================
# Purpose: simple Makefile to streamline processing latex document (just say "make" to execute)
# Author: Tomasz Skwarnicki
# Created on: 2010-09-24
# A few changes by Patrick Koppenburg on 2015-06-26
# ===============================================================================

# name of the main latex file (do not include .tex)
MAIN = main

# name of the target - change that to something descriptive, like paper-v0, Bs2PhiPhi-ANA-v1, etc...
TARGET = template

# name of command to perform Latex (either pdflatex or latex)
LATEX = pdflatex

ifeq ($(LATEX),pdflatex)
	FIGEXT = .pdf
	MAINEXT= .pdf
	BUILDCOMMAND=rm -f $(MAIN).aux && $(LATEX) $(MAIN) && bibtex $(MAIN) && $(LATEX) $(MAIN) && $(LATEX) $(MAIN)
	BUILDCOMMANDPRL=rm -f $(MAIN)-prl.aux && $(LATEX) $(MAIN)-prl && bibtex $(MAIN)-prl && $(LATEX) $(MAIN)-prl && $(LATEX) $(MAIN)-prl
	MAKEMAINCOUNT= sed 's\#{wordcount}{false}\#{wordcount}{true}\#' main-prl.tex > main-count.tex
	BUILDCOMMANDCOUNT= $(MAKEMAINCOUNT) && rm -f $(MAIN)-count.aux && $(LATEX) $(MAIN)-count && bibtex $(MAIN)-count >/dev/null; true && $(LATEX) $(MAIN)-count && ./wordcount.sh $(MAIN)-count && rm wordcount.pdf main-count* 
else
	FIGEXT = .eps
	MAINEXT= .pdf
	BUILDCOMMAND=rm -f $(MAIN).aux && $(LATEX) $(MAIN) && bibtex $(MAIN) && $(LATEX) $(MAIN) && $(LATEX) $(MAIN) && dvips -z -o $(MAIN).ps $(MAIN) && ps2pdf $(MAIN).ps && rm -f head.tmp body.tmp
	BUILDCOMMANDPRL=rm -f $(MAIN)-prl.aux && $(LATEX) $(MAIN)-prl && bibtex $(MAIN)-prl && $(LATEX) $(MAIN)-prl && $(LATEX) $(MAIN)-prl && dvips -z -o $(MAIN)-prl.ps $(MAIN)-prl && ps2pdf $(MAIN)-prl.ps && rm -f head.tmp body.tmp
	BUILDCOMMANDCOUNT=
endif

# list of all source files
TEXSOURCES = $(wildcard *.tex) $(wildcard *.bib)
FIGSOURCES = $(wildcard figs/*$(FIGEXT))
SOURCES    = $(TEXSOURCES) $(FIGSOURCES)

# define output (could be making .ps instead)
OUTPUT = $(TARGET)$(MAINEXT)

# cp temporary main.pdf to target.
$(OUTPUT): $(MAIN)$(MAINEXT)
	cp $(MAIN)$(MAINEXT) $(OUTPUT)

# prescription how to make output (your favorite commands to process latex)
# do latex twice to make sure that all cross-references are updated 
$(MAIN)$(MAINEXT): $(SOURCES) Makefile
	$(BUILDCOMMAND)

# just so we can say "make all" without knowing the output name
all: $(OUTPUT)

# remove temporary files (good idea to say "make clean" before putting things back into repository)
.PHONY : clean
clean:
	rm -f *~ *.aux *.log *.bbl *.blg *.dvi *.tmp *.out *.blg *.bbl $(OUTPUT) $(MAIN)$(MAINEXT) $(MAIN).ps $(MAIN)-prl.ps $(MAIN)-prlNotes.bib

# remove output file
rmout: 
	rm $(OUTPUT) $(MAIN)$(MAINEXT)

# Make the PRL version
prl: 
	$(BUILDCOMMANDPRL)

# Make the PRL version
count: 
	$(BUILDCOMMANDCOUNT)
	@echo ''
	@echo 'Figures:   Add 20+150/(aspect ratio) per figure'
	@echo 'Equations: Add 16 words per row (single column) '
	@echo 'Tables:    Add 13 words plus 6.5 words per line (single column)'
	@echo 

